winPIBT: Extended Prioritized Algorithm for Iterative Multi-agent Path Finding

The problem of Multi-agent Path Finding (MAPF) consists in providing agents with efficient paths while preventing collisions. Numerous solvers have been developed so far since MAPF is critical for practical applications such as automated warehouses. The recently-proposed Priority Inheritance with Backtracking (PIBT) is a promising decoupled method that solves MAPF iteratively with flexible priorities. The method is aimed to be decentralized and has a very low computational cost, but it is shortsighted in the sense that it plans only one step ahead, thus occasionally resulting in inefficient plannings. This work proposes a generalization of PIBT, called windowed PIBT (winPIBT), that introduces a configurable time window. winPIBT allows agents to plan paths anticipating multiple steps ahead. We prove that, similarly to PIBT, all agents reach their own destinations in finite time as long as the environment is a graph with adequate properties, e.g., biconnected. Experimental results over various scenarios confirm that winPIBT mitigates livelock situations occurring in PIBT, and usually plans more efficient paths given adequate window size.

==> table/large-mapf.tex <==
\begin{figure*}
 \centering
  \begin{tabular}{ccc}
   \begin{minipage}[t]{0.33\hsize}
    \centering
    \includegraphics[width=1\hsize]{fig/8x8_path.pdf}
   \end{minipage}
   \begin{minipage}[t]{0.33\hsize}
    \centering
    \includegraphics[width=1\hsize]{fig/8x8_success.pdf}
    \subcaption{$8\stimes 8$}
   \end{minipage}
   \begin{minipage}[t]{0.33\hsize}
    \centering
    \includegraphics[width=1\hsize]{fig/8x8_runtime.pdf}
   \end{minipage}
   \vspace{0.2cm}
   \\
   \begin{minipage}[t]{0.33\hsize}
    \centering
    \includegraphics[width=1\hsize]{fig/ca_caverns1_path.pdf}
   \end{minipage}
   \begin{minipage}[t]{0.33\hsize}
    \centering
    \includegraphics[width=1\hsize]{fig/ca_caverns1_success.pdf}
    \subcaption{ca\_caverns1}
   \end{minipage}
   \begin{minipage}[t]{0.33\hsize}
    \centering
    \includegraphics[width=1\hsize]{fig/ca_caverns1_runtime.pdf}
   \end{minipage}
   \end{tabular}
 \vspace{-0.1cm}
 \caption{Results of one-shot MAPF.
 From the left, each figure corresponds to ``path'', ``success'' and ``runtime'', respectively.
 Error bars correspond to standard errors.
 }
 \label{fig:large-mapf}
\end{figure*}

==> table/naive.tex <==
\setlength{\tabcolsep}{1.2mm}
\renewcommand{\arraystretch}{1.1}
\begin{table}
 \centering
 \caption{
 The results of \naive iterative MAPF.
 }
 \label{table:naive}
 \vspace{-0.25cm}
 \small{
 \begin{tabular}{c|c|l|r|r|r}
  \toprule
  field & \begin{tabular}{c} agents/\\tasks \end{tabular}
  & solver & makespan & \begin{tabular}{c} service\\time \end{tabular} & runtime {\tiny (s)} \\ \hline
  & & \winpibt-2 & 770.9 & 67.6 & 4  \\ \cline{3-6}
  & & \winpibt-3 & 769.4 & 67.3 & 5 \\ \cline{3-6}
  & & \winpibt-5 & \textbf{761.3} & \textbf{66.9} & 5 \\ \cline{3-6}
  \floor & 100/1000 & \winpibt-7 & 765.1 & 67.2 & 6 \\ \cline{3-6}
  & & \winpibt-10 & 769.1 & 68.0 & 7 \\ \cline{3-6}
  & & \winpibt-15 & 778.0 & 68.5 & 10 \\ \hhline{~|~|=|=|=|=}
  & & PIBT & 780.2 & 67.8 & 1 \\ \midrule
  %
  & & \winpibt-2 & \textbf{1967.6} & \textbf{176.2} & 465 \\ \cline{3-6}
  & & \winpibt-3 & 1983.3 & 177.5 & 488 \\ \cline{3-6}
  & & \winpibt-5 & 2003.5 & 178.7 & 503 \\ \cline{3-6}
  \textit{magic} & 500/5000 & \winpibt-7 & 2015.3 & 180.0 & 525 \\ \cline{3-6}
  \textit{roundabout} & & \winpibt-10 & 2030.6 & 180.7 & 563 \\ \cline{3-6}
  & & \winpibt-15 & 2052.4 & 182.0 & 649 \\ \hhline{~|~|=|=|=|=}
  & & PIBT & 1970.9 & 176.5 & 25 \\
  \bottomrule
 \end{tabular}
 }
\end{table}

==> table/small-mapf.tex <==
\setlength{\tabcolsep}{1.2mm}
\renewcommand{\arraystretch}{1.1}
\begin{table}[b]
 \centering
 \caption{
 The results of one-shot MAPF.
 }
 \label{table:small-mapf}
 \vspace{-0.25cm}
 \small{
 \begin{tabular}{c|c|l|r|r|r}
  \toprule
  field & agents & solver & path & success & runtime {\tiny (ms)} \\ \midrule
  & & \winpibt-2 & 11.9 &  99 & 0 \\ \cline{3-6}
  & & \winpibt-3 & 12.1 & \textbf{100} & 0 \\ \cline{3-6}
  & & \winpibt-4 & \textbf{11.9} & \textbf{100} & 0 \\ \cline{3-6}
  \bridge & 4 & \winpibt-5 & 12.2 & \textbf{100} & 0 \\ \cline{3-6}
  & & \winpibt-10 & 13.7 & \textbf{100} & 1 \\ \hhline{~|~|=|=|=|=}
  & & PIBT & 11.4 & 100 & 0 \\ \cline{3-6}
  & & CBS & 7.8 & 89 & 18438 \\ \midrule
  %
  & & \winpibt-2 & 7.3 & 65 & 0 \\ \cline{3-6}
  & & \winpibt-3 & \textbf{6.9} & 64 & 0 \\ \cline{3-6}
  & & \winpibt-5 & 7.4 & 73 & 0 \\ \cline{3-6}
  \twoloop & 4 & \winpibt-7 & 7.0 & 74 & 0 \\ \cline{3-6}
  & & \winpibt-10 &  9.7 & 93 & 1 \\ \cline{3-6}
  & & \winpibt-15 & 11.9 & \textbf{97} & 2 \\ \hhline{~|~|=|=|=|=}
  & & PIBT & 7.6 & 55  & 0 \\ \cline{3-6}
  & & CBS  & 5.0 & 100 & 658 \\ \midrule
  %
  & & \winpibt-2 & \textbf{6.3} & 73 & 0 \\ \cline{3-6}
  & & \winpibt-3 & 6.7 & 72 & 0 \\ \cline{3-6}
  & & \winpibt-5 & 6.7 & 73 & 0 \\ \cline{3-6}
  \twolooprest & 5 & \winpibt-7 & 7.8 & 82 & 0 \\ \cline{3-6}
  & & \winpibt-10 & 8.4 & 94 & 1 \\ \cline{3-6}
  & & \winpibt-15 & 9.2 & \textbf{97} & 2 \\ \hhline{~|~|=|=|=|=}
  & & PIBT & 7.1 & 70 & 0   \\ \cline{3-6}
  & & CBS  & 5.0 & 99 & 273 \\ \midrule
  %
  & & \winpibt-5  & 105.8 & \textbf{100} & 914 \\ \cline{3-6}
  & & \winpibt-15 & 102.3 & \textbf{100} & 1846 \\ \cline{3-6}
  \kivalike & 100 & \winpibt-30 & 99.5 & \textbf{100} & 9595 \\ \cline{3-6}
  & & \winpibt-50 & \textbf{96.0} & \textbf{100} & 48274 \\ \hhline{~|~|=|=|=|=}
  & & PIBT & 103.6 & 33 & 110 \\ \cline{3-6}
  & & iECBS (1.2) & 62.2 & 72 & 109827 \\
  %
  \bottomrule
 \end{tabular}
 }
\end{table}

==> tikz/naive-benchmarks.tex <==
\begin{figure}
 \centering
 \begin{tabular}{c}
  \begin{minipage}[t]{1\hsize}
   \centering
   \includegraphics[width=1\hsize]{fig/8f.pdf}
   \vspace{-0.5cm}
   \subcaption{\floor ($135\stimes 21$)}
   \label{fig:naive:floor}
  \end{minipage}
  \vspace{0.2cm}
  \\
  \begin{minipage}[t]{1\hsize}
   \centering
   \begin{tikzpicture}
    \node[anchor=south west,inner sep=0] at (0,0)
    {\includegraphics[width=1\hsize]{fig/magic-roundabout-arrow.pdf}};
    \node[anchor=west] at (0.5, 4.7) {\textcolor{white}{\scriptsize area A}};
    \node[anchor=west] at (3.9, 4.8) {\textcolor{white}{\scriptsize area B}};
    \node[anchor=west] at (7.0, 4.4) {\textcolor{white}{\scriptsize area C}};
    \node[anchor=west] at (0.6, 2.8) {\textcolor{white}{\scriptsize area D}};
    \node[anchor=west] at (7.5, 3) {\textcolor{white}{\scriptsize area E}};
    \node[anchor=west] at (3.0, 0.8) {\textcolor{white}{\scriptsize area F}};
   \end{tikzpicture}
   \vspace{-0.5cm}
   \subcaption{\mra ($160\stimes 100$)}
   \label{fig:naive:mra}
  \end{minipage}
 \end{tabular}
 \caption{Benchmarks for \naive iterative MAPF.}
 \label{fig:naive}
\end{figure}
